ERNIE-Tiny : A Progressive Distillation Framework for Pretrained Transformer Compression

Pretrained language models (PLMs) such as BERT adopt a training paradigm which first pretrain the model in general data and then finetune the model on task-specific data, and have recently achieved great success. However, PLMs are notorious for their enormous parameters and hard to be deployed on real-life applications. Knowledge distillation has been prevailing to address this problem by transferring knowledge from a large teacher to a much smaller student over a set of data. We argue that the selection of thee three key components, namely teacher, training data, and learning objective, is crucial to the effectiveness of distillation. We, therefore, propose a four-stage progressive distillation framework ERNIE-Tiny to compress PLM, which varies the three components gradually from general level to task-specific level. Specifically, the first stage, General Distillation, performs distillation with guidance from pretrained teacher, gerenal data and latent distillation loss. Then, General-Enhanced Distillation changes teacher model from pretrained teacher to finetuned teacher. After that, Task-Adaptive Distillation shifts training data from general data to task-specific data. In the end, Task-Specific Distillation, adds two additional losses, namely Soft-Label and Hard-Label loss onto the last stage. Empirical results demonstrate the effectiveness of our framework and generalization gain brought by ERNIE-Tiny.In particular, experiments show that a 4-layer ERNIE-Tiny maintains over 98.0%performance of its 12-layer teacher BERT base on GLUE benchmark, surpassing state-of-the-art (SOTA) by 1.0% GLUE score with the same amount of parameters. Moreover, ERNIE-Tiny achieves a new compression SOTA on five Chinese NLP tasks, outperforming BERT base by 0.4% accuracy with 7.5x fewer parameters and9.4x faster inference speed.

==> nips/fig/old_performance_comparsion.tex <==

\begin{figure}[htbp]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{nips/tiny-4-3-a-fit.pdf}
        \caption{Performance of Different Compression Methods}
        \label{fig:tiny-a}
     \end{subfigure}
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{nips/tiny-4-3-b-fit.pdf}
         \caption{Effectiveness of each stage}
         \label{fig:tiny-b}
     \end{subfigure}

     \vspace{-7mm}
\end{figure}


==> nips/sec/checklist.tex <==
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Conclusion.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We have released our code on github.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{sec:experiment_setup} and the Appendix.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{We do not report error bars. Experiment results in ablation study are an average of 5 runs with a different random seed. }
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We use GLUE datset for validation and cite it in Section 4.1.1}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{We use open source data and follow their licenses.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{We do not use these data.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> nips/sec/old_experiment.tex <==
	\section{Experiment}
To fully study the proposed ERNIE-Tiny framework, we perform empirical studies on the several datasets, and compare our distillation results with the strong baseline methods.
	
	\subsection{Experiment Setup}
	For fair comparison, we adopt pretrained BERT${}_{base}$ checkpoint release by the author and finetuned a BERT${}_{base}$ model for each task, and pick the best dev-set performance model as the teacher. 
	The BERT${}_{base}$ teacher in our experiment has 12 Transformer layers, 768 hidden size and 3076 intermediate hidden size, accounting for 109M of parameters in total. 
	
	
	For the same reason of fair comparison with other approaches, we choose a student Transformer of 4 layers, 312 hidden size and 1200 intermediate hidden size. 
	For the proposed GED, we perform 500K steps of parameter updates with a batch size of 1280. To adapt unsupervised corpus to text pair input teacher model, we construct a input pair by sampling consecutive text pairs in unsupervised corpus. To ensure no additional resource or knowledge is used in GED, we only use English Wikipedia and BooksCorpus as it is used in \cite{devlin2018bert}.
	

	\begin{table}[hbp]
		\centering
		\scalebox{0.8}{
			\begin{tabular}{ l|ccccc}
				\toprule
				Method          & MNLI(m/mm)             & RTE              & MRPC                    & CoLA        & Ave \\
				\midrule
				BERT${}_{Base}$ (T.)             & 84.5/84.6          &  69.7          & 86.8                  & 61.3  & 77.4    \\
				ERNIE-Tiny (w/o GD GED)    & 63.9/63.6          &  53.4          & 68.9          & 23.5	& 62.5   \\
				ERNIE-Tiny (w/o GED)    & 82.4/82.4          &  66.4          & 86.1           & 49.2	& 73.3    \\
				ERNIE-Tiny (w/o GD)   & 83.0/83.1 &  67.1 & 86.4           & 49.1   &73.7  \\
				ERNIE-Tiny & 83.0/83.0          &  66.8          & 86.9 & 50.0 & 73.9    \\
				\bottomrule
			\end{tabular}
		}
		\caption{Ablation study on distillation with general data}
		\label{tab:ablation1}
	\end{table}
	\begin{table}[htp]
		\centering
		\begin{tabular}{ l|ccccc } 
			\toprule
			Method & MNLI(m/mm)         & RTE           & MRPC         &   CoLA & Ave  \\
			\midrule
			GD+GED+TAD+TD    &83.0/83.0 &66.8         &86.9 &  50.0 & 73.9 \\ 
			GD+GED+TD        &81.2/81.5 &69.0         &     86.3   &  37.4 & 71.1\\ 
			GD+GED+FT directly   &80.7/81.2 &66.5         &79.8 &  0.0 &61.6      \\ 
			\bottomrule
		\end{tabular}
		\caption{Ablation study on distillation with task-specific data}
		\label{tab:ablation3}
	\end{table}
	
	
	\begin{table}[htbp]
		\centering
		\begin{tabular}{ r|rrr }
			\toprule
			proportion  & MNLI  & QNLI  & QQP      \\
			\midrule
			1\%         & 3927  & 1047  & 3638      \\
			10\%        & 39270 & 10474 & 36384     \\
			50\%        & 196351& 52371 & 181925    \\
			\bottomrule
		\end{tabular}
		\caption{Number of labeled data for ablation study}
		\label{tab:ablation2-1}
	\end{table}
	
	\begin{table}[htbp]
		\begin{tabular}{ l|ccc|c }
			\toprule
			Method                           & MNLI(m/mm)         & QNLI         & QQP    & Ave  \\
			\midrule
			\multicolumn{4}{l}{1\% of labeled data}                                             \\
			\hline
			BERT${}_{base}$ (T.)           & 67.0/69.3       & 78.4       & 71.3  & 71.5\\
			ERNIE-Tiny(w/o GED)                   & 57.7/60.5	 & 75.4       & 69.4 & 65.8  \\
			ERNIE-Tiny(w/ GED)                   & 65.2/67.4     & 75.4       & 70.8  & 69.7 \\
			gain of GED                          &  +7.5/+6.8       & +0.0       & +1.4 & +4.1  \\
			\midrule
			\multicolumn{4}{l}{10\% of labeled data}                                             \\
			\hline
			BERT${}_{base}$ (T.)            & 76.4/77.3	     & 86.9       & 79.7  & 80.1 \\
			ERNIE-Tiny(w/o GED)                   & 69.1/69.8      & 82.4       & 78.2 & 74.9  \\
			ERNIE-Tiny(w/ GED)                 & 74.5/75.0      & 82.4	    & 78.1 &77.5 \\
			gain of GED                           & +5.5/+5.2       & +0.0        & -0.1  & +2.6  \\
			\midrule
			\multicolumn{4}{l}{50\% of labeled data}                                             \\
			\hline
			BERT${}_{base}$ (T.)            & 80.5/81.9	     & 90.1       & 84.2  & 84.2 \\
			ERNIE-Tiny(w/o GED)                  & 75.3/76.4	     & 83.5       & 83.3 & 79.6  \\
			ERNIE-Tiny(w/ GED)                   & 79.3/80.1	     & 84.2       & 83.5  & 81.8 \\
			gain of GED                           & +4.0/+3.7       & +0.8       & +0.2   & +2.2  \\
			\bottomrule
		\end{tabular}
		\caption{Ablation study on labeled data size}
		\label{tab:ablation2}
	\end{table}
	\begin{table*}[htbp]
		\begin{tabular}{ l|cccc|c }
			\toprule
			Method                        & MNLI(m/mm)   & RTE   & MRPC  & CoLA  & Ave \\ \midrule
			BERT${}_{Base}$ (L=12;h=768;d=3072) (T.)            & 84.4/84.6  & 69.7 & 86.7 & 61.3 & 77.3 \\
			\midrule 
			ERNIE-Tiny (L=4;h=312;d=1200)   & 82.4/82.4  & 66.8 & 86.4 & 50.0 & 73.6 (-3.7)      \\ 
			ERNIE-Tiny (L=12;h=768;d=3072)  & 84.6/84.9  & 72.3 & 87.3 & 62.1 & 78.2 (+0.9)          \\ 
			\bottomrule
		\end{tabular}
		\caption{Ablation study on student capacity}
		\label{tab:ablation4}
	\end{table*}
	
	
	\begin{table*}[htbp]
		\begin{tabular}{ l|cccc|c }
			\toprule
			Method                                    &     STS-B   & SST-2 & RTE  & CoLA & Ave  \\
			\midrule 
			ERNIE-Tiny (w/ TinyBERT styled data-augment)      &     87.2    & 92.7  & 66.8 & 50.0 & 74.1 \\ 
			ERNIE-Tiny (w/ extra transfer distillation)       &     88.2    & 93.3  & 70.0 & 53.2 & 76.1\\  
			\bottomrule
		\end{tabular}
		\caption{Ablation study on extra transfer distillation}
		\label{tab:ablation5}
	\end{table*}	
	
	
	\begin{table*}
		\begin{center}
			\scalebox{0.75}{
				\begin{tabular}{
						l|c|c|ccccc|c
					}
					\toprule
					Method   & Params  & Speedup     & XNLI   & LCQMC  & ChnSentiCorp     & NLPCC-DBQA  & MSRA-NER  & Ave      \\
					\midrule
					ERNIE2.0${}_{Base}$ (T.) & 109M& 1x &79.8 & 87.5 & 95.5 & 84.4 & 95.0 & 88.4 \\
					\midrule
					BERT${}_{Base}$ & 109M & 1x &77.2 & 87.0 & 94.3 & 80.9 & 92.3 & 86.3   \\
					ERNIE-Tiny & \textbf{14.5M} & \textbf{9.4x} & \textbf{77.6} & \textbf{88.0} & \textbf{94.9} & \textbf{82.2} & \textbf{90.8} &  \textbf{86.7} \\
					\bottomrule
				\end{tabular}
			}
			\caption{The Test Results of Chinese Tasks. TinyBERT on this table is reproducted by us. Both TinyBERT and our model are 4-layer Transformer with 312 hidden size and 1200 intermedia hidden size and the teacher is set to ERNIE2.0$_{base}$ for fairness. The state-of-the-art results are in bold.}
		    \label{tab:chinese}
		    
		\end{center}
	\end{table*}
 
 \subsection{English ERNIE-Tiny}
\subsubsection{Downstream Tasks}
GLUE \cite{glue} is a well-studied collection of NLP tasks, including textual entailment, emotion detection, coreference resolution, etc. 
In detail, we choose to evaluate our model in 8 tasks, namely Multi-Genre Language Inference(MNLI), Question Natual Language Inference(QNLI), Quora Question Paris (QQP),  Standford Sentiment Treebank(SST-2),  Semantic Textual Similarity Benchmark(STS-b), Corpus of Linguistic Acceptability(CoLA), Recognizing Textual Entailment(RTE), and Microsoft Research Paragraph Corpus(MRPC).
Following \cite{devlin2018bert},  we cast these tasks to sentence pair classification problem and evaluate the distilled model with metrics use by GLUE, all tasks use accuracy as metrics except for MRPC(F1-score), QQP(F1-score) and STS-b(Matthew’s correlation).  We report test-set results evaluated by GLUE server in our main results, and dev-set results in the ablation studies. 
	In TAD, since some of the tasks like RTE and CoLA contains very limited resource for distillation training, the data augment procedure proposed in TinyBERT \cite{tinybert} has become a common practice for in model distillation. For fair comparison, we perform the same data augment procedure in our ablation studies. 
	However when submit to GLUE test server, we perform an extra transfer distillation stage before TAD on low resource tasks like MRPC, STS-B, SST2, CoLA and RTE, we use MNLI as transfer dataset and perform transfer distillation with batch size 256 sequence and learning rate 1e-4 for 20 epoch. This utilization of MNLI dataset to extends low-resource task was first introduced by \cite{roberta}, note that we do not incorporate this trick in the finetuning of our teacher model.
	
	TAD utilizes only latent distillation, with batch size 256 sequence and learning rate 5e-5 for 5 epochs on larger dataset like MNLI/QNLI/QQP and batch size 32 sequences, learning rate 5e-5 for 10 epoch on smaller dataset like SST-2/STS-B/RTE. Especially, we perform 50 epoch on CoLA for TAD. 
	Both prediction distillation and latent distillation are utilized in TD, with batch size 256 sequences for MNLI/QNLI/QQP  and batch size 32 sequences for  SST-2/STS-B/RTE, all tasks share stage2 learning rate 3e-5 and 3 training epoch.
	We conduct our experiment on 8 V100 GPUs for GD and GED, and 1-4 V100 GPUs for TAD and TD. The reported dev-set metrics are an average of 5 runs with a different random seed.

	\subsubsection{Main Results}
	We demonstrate our results on the test set of GLUE and compare them with other compression models on Table \ref{tab:glue}. 
	It can be seen that our model is more effective than BERT-PKD and DistillBert. Also, our model exceeds TinyBERT by 1.0\% average score, and is improved on almost every GLUE task.
	MobileBERT use IB-BERT teacher model, which has the same model size with BERT${}_{large}$. If we use BERT${}_{large}$ as teacher model, we can have better result.
	MiniLM does not have task-specific distillation, which is more convenient to use, but the performance is not as good as that with task-specific distillation. For fairness, we mainly compare the proposed method with task-specific distillation methods in this paper.
	
	
	\subsubsection{Ablation Studies}
	We perform ablation studies on the key factors to evaluate the contribution of each component to overall performance, including general data based distillation stages and task-specific data based distillation stages. Intensive experiments conclude the effect of our curriculum learning framework is more obvious when labeled data set is small. In addition, we also designed experiments to observe the performance when the student reaches the same size as the teacher. All results on GLUE in ablation studies is on DEV set.
	
	\textbf{Effect of General Data based Distillation}
	We perform ablation studies of using the unsupervised general data on 3 low-resource tasks MRPC/RTE/CoLA and 1 high-resource task MNLI. 
	As introduced earlier, general data is only utilized for task-agnostic distillation in GD and task-specific distillation in GED, so we try 4 kinds of distillation with the pretraining general data: 1) do not use the general data; 2) latent represent distillation of pretrained BERT${}_{base}$ as the teacher for 1M steps in GD; 3) latent represent distillation of finetuned BERT${}_{base}$ for 500K steps in GED; 4) combination of 2) and 3). 
	After that, all four experiments perform the same distillation using task-specific data to evaluate the final performances.
	As it is shown in Table \ref{tab:ablation1}, the distillation is very poor without general data. Distillation from finetuned teacher in GED perform better than distillation from pretrained teacher in GD. For NLI tasks like RTE and MNLI, the additional task-agnostic distillation hurts performance. For other tasks, the combination of both distillations yields better results.
	
	\textbf{Effect of Task-specific Data based Distillation}
	The proposed TAD shares the same distillation loss as GED but has different transfer data. 
	To verify if these two stages are complementary to each other, we varied the distillation objective in the task-specific data distillation stage. 
	As it is shown in Table \ref{tab:ablation3}, we choose to remove TAD and finds performance degradation. 
	We try to solely finetune our student model with the gold label, which also leads to a performance drop. This indicates that latent distillation on task-specific data is non-negligible and should be combined with general distillation.
	
	\textbf{Effect of Labeled Dataset Size}
	The pretraining corpus introduced in the task-specific distillation stage can be regarded as a supplement to the original task dataset, which is more effective on low-resource tasks. 
	To illustrate this, we varied the labeled dataset size of MNLI, QNLI and QQP tasks to 1\%, 10\% and 50\% of the original size, the resulting data size is listed inTable \ref{tab:ablation2-1}. Then we finetune BERT$_{base}$ teacher for each configuration and perform task-specific distillation from the stretch. 
	Results are presented in Table \ref{tab:ablation2}, from which we can see that teacher performance degrades severely when only fed 1\% of training label, and GED achieves larger performance gain on low-resource settings.
	
	\textbf{Effect of Student Capacity}
	We show the effect of student models with different parameters, including the same size as teacher model. It also be called self-training. 
	Both of our models distill from BERT${}_{base}$. Interestingly, we found that through self-training distillation, we could significantly improve the effectiveness of the model with the original model size.
	The student model exceeds teacher 0.9\% average score.
	
	\textbf{Effect of Extra Transfer Distillation}
	As described in experiment setup, we introduce an extra transfer distillation stage for low-resource tasks. We discard the label of MNLI training data and used it directly in latent distillation of sentence pair Tasks. For classification task of single sentence, the sentence pair from MNLI training data is split and treated as two independent sentence input. The performance gain of 20 epoch of extra distillation is presented in Table \ref{tab:ablation5}. It can be seen that tasks with lower performance like CoLA benefits most from transfer distillation.
	
	\subsection{Chinese ERNIE-Tiny}
	Since most of the compression models do not have public effects on Chinese tasks and open source models, we reproduct TinyBERT for comparing. Both TinyBERT and our model is distilled from an ERNIE2.0${}_{base}$ model, using the same pretraining data. 
	BERT${}_{base}$ is the baseline for comparison. 
	We executed extensive experiments on 5 Chinese NLP tasks, including natural language inference, semantic similarity, sentiment analysis and question answering and named entity recognition. Some of them use sentence-pair as inputs.
	
	\textbf{Single Sentence Tasks}  
	\begin{itemize}
            \item Sentiment Analysis (SA): ChnSentiCorp
            \item Named Entity Recognition (NER): MSRA-NER
	\end{itemize}

	\textbf{Sentence pair Tasks}
	\begin{itemize}
		\item Question Answering (QA): NLPCC-DBQA
		\item Semantic Similarity (SS): LCQMC
		\item Natural Language Inference (NLI): XNLI
	\end{itemize}
	
	The test result of each model is on Table \ref{tab:chinese}. It can be seen that ERNIE2.0${}_{Base}$ outperforms BERT${}_{Base}$ on all five tasks. Our model distill from ERNIE2.0${}_{Base}$ by our ERNIE-Tiny framework outperforms BERT${}_{Base}$ on XNLI, LCQMC, ChnSentiCorp and NLPCC-DBQA tasks and exceeds it by 0.4\% average score on five tasks, while it has 7.5x smaller parameters and 9.4x average score. We also fint that the tiny model is not good at a token-level task like NER, which has a 4.16\% score gap between the teacher and student model.
	
	\subsection{Discussion}
	 

\section{Conclusion}
In this paper, we propose a four-stage ERNIE-Tiny framework via curriculum learning. Unsupervised pretraining corpus is utilized in task-specific distillation, making our training more smooth. 
Through extensive empirical study, we show that our ERNIE-Tiny framework not only leads to better distillation performance on the compact model but also improves performance in self-training scenario. 
Task-specific distillation requires relatively longer training time when adapting to multiple downstream tasks, acceleration of this procedure on a much larger teacher like Albert-large with other techniques like quantization or pruning is left for future work.

==> nips/tbl/data_aug.tex <==
	\begin{table*}[htbp]
		\begin{tabular}{ l|cccc|c }
			\toprule
			Method                                    &     STS-B   & SST-2 & RTE  & CoLA & Avg.  \\
			\midrule 
			ERNIE-Tiny (w/ TinyBERT styled data-augment)      &     87.2    & 92.7  & 66.8 & 50.0 & 74.1 \\ 
			ERNIE-Tiny (w/ extra transfer distillation)       &     88.2    & 93.3  & 70.0 & 53.2 & 76.1\\  
			\bottomrule
		\end{tabular}
		\caption{Ablation study on extra transfer distillation}
		\label{tab:data_aug}
	\end{table*}

==> nips/tbl/datasize.tex <==
	\begin{table}[htbp]
		\centering
		\begin{tabular}{ r|rrr }
			\toprule
			proportion  & MNLI  & QNLI  & QQP      \\
			\midrule
			1\%         & 3927  & 1047  & 3638      \\
			10\%        & 39270 & 10474 & 36384     \\
			50\%        & 196351& 52371 & 181925    \\
			\bottomrule
		\end{tabular}
		\caption{Number of labeled data for ablation study}
		\label{tab:datasize}
	\end{table}

==> nips/tbl/datasize_performance.tex <==
	\begin{table}[htbp]
	\centering
	\scalebox{0.6}{
		\begin{tabular}{ l|cccc|c }
			\toprule
			Method                           & MNLIm & MNLImm         & QNLI         & QQP    & Avg.  \\
			\midrule
			\multicolumn{4}{l}{1\% of labeled data}                                             \\
			\hline
			BERT${}_{base}$ (T.)           & 67.0 & 69.3       & 78.4       & 71.3  & 71.5\\
			ERNIE-Tiny(w/o GED)                   & 57.7& 60.5	 & 75.4       & 69.4 & 65.8  \\
			ERNIE-Tiny(w/ GED)                   & 65.2 & 67.4     & 75.4       & 70.8  & 69.7 \\
			gain of GED                          &  +7.5& +6.8       & +0.0       & +1.4 & +4.1  \\
			\midrule
			\multicolumn{4}{l}{10\% of labeled data}                                             \\
			\hline
			BERT${}_{base}$ (T.)            & 76.4&77.3	     & 86.9       & 79.7  & 80.1 \\
			ERNIE-Tiny(w/o GED)                   & 69.1&69.8      & 82.4       & 78.2 & 74.9  \\
			ERNIE-Tiny(w/ GED)                 & 74.5&75.0      & 82.4	    & 78.1 &77.5 \\
			gain of GED                           & +5.5&+5.2       & +0.0        & -0.1  & +2.6  \\
			\midrule
			\multicolumn{4}{l}{50\% of labeled data}                                             \\
			\hline
			BERT${}_{base}$ (T.)            & 80.5&81.9	     & 90.1       & 84.2  & 84.2 \\
			ERNIE-Tiny(w/o GED)                  & 75.3&76.4	     & 83.5       & 83.3 & 79.6  \\
			ERNIE-Tiny(w/ GED)                   & 79.3&80.1	     & 84.2       & 83.5  & 81.8 \\
			gain of GED                           & +4.0&+3.7       & +0.8       & +0.2   & +2.2  \\
			\bottomrule
		\end{tabular}
		}
		\vspace{1mm}
		\caption{Ablation study on labeled data size}
		\label{tab:datasize_performance}
	\end{table}
	\vspace{-7mm}

==> nips/tbl/glue_results_old.tex <==
\begin{table*}[htbp]
	\centering
	\scalebox{0.7}{
			\begin{tabular}{
					ccccccccccccc }
				\toprule
				Method         &Params  &Speedup          & MNLIm & MNLImm & QQP & SST-2 & QNLI & MRPC & RTE & CoLA & STS-B &  Ave \\ 
				\midrule
				BERT${}_{Base}$(T.)   & 109M    &1x   & 84.6 & 83.4 & 71.2 & 93.5 & 90.5 & 88.9 & 66.4 & 52.1 & 85.8 & 79.6\\ 
				\midrule
				BERT-PKD              & 52.2M    &2x    & 79.9 & 79.3 & 70.2 & 89.4 & 85.1 & 82.6 & 62.3 & 24.8 & 79.8 & 72.6 \\
				DistillBERT  & 52.2M         &2x        & 78.9 & 78.0 & 68.5 & 91.4 & 85.2 & 82.4 & 54.1 & 32.8 & 76.1 & 71.9 \\
				BERT-EMD 	 & 14.5M  &9.4x          & 82.1 & 80.6 & 69.3 & 91.0 & 87.2 & 87.6 & 66.2 & 25.6 & \textbf{82.3} & 74.6 \\
				MobileBERT* & 15.1M &8.6 x &  81.5 & 81.6 & 68.9 & 91.7 & \textbf{89.5} & 87.9 & 65.1 &  46.7 & 80.1 &  77.0 \\ 
				TinyBERT          & 14.5M  &9.4x          & 82.5 & \textbf{81.8} & \textbf{71.3} & 92.6 & 87.7 & 86.4 & \textbf{66.6} & 44.9 & 80.4 & 77.0\\ 
				ERNIE-Tiny       & \textbf{14.5M}  &\textbf{9.4x}           & \textbf{83.0} & \textbf{81.8} & \textbf{71.3} & \textbf{93.3}    & 88.3 & \textbf{88.4} & \textbf{66.6} & \textbf{47.4} & \textbf{82.3} & \textbf{78.0} \\
				\bottomrule
			\end{tabular}
	}
	\caption{GLUE test results that are scored by GLUE evaluation server. The state-of-the-art results are in bold. BERT$_{base}$ is the teacher model of most methods, except MobileBERT. MobileBERT is distilled from IB-BERT, which has the same model size with BERT${}_{large}$, so comparison may not be fair. 
	The architecture of ERNIE-Tiny, BERT-EMD and TinyBERT is (${L}$=4, ${h}$=312, ${d}$=1200), BERT-PKD and DistilBERT is (${L}$=4, ${h}$=768, ${d}$=3072). MobileBERT is (${L}$=24, ${h}$=128, ${d}$=512).
	}
	\label{tab:glue}
\end{table*}

==> nips/tbl/ood-datasize.tex <==
\begin{table}[!htb]
\begin{minipage}{.5\linewidth}
		\centering
		\begin{tabular}{ r|rrr }
			\toprule
			proportion  & MNLI  & QNLI  & QQP      \\
			\midrule
			1\%         & 3927  & 1047  & 3638      \\
			10\%        & 39270 & 10474 & 36384     \\
			50\%        & 196351& 52371 & 181925    \\
			\bottomrule
		\end{tabular}
		\vspace{1mm}
		\caption{Number of labeled data for ablation study}
		\label{tab:datasize}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
		\begin{tabular}{l|c|cc}
			\toprule
			method                                 &     MNLIm   & SNLI & RTE  \\
			\midrule 
			GD+GED+TSD      &    81.2     & 75.9  & 65.7 \\ 
			GD+TAD+TSD       &  82.4 & 70.9 & 52.8\\  
            GD+TSD       &   80.8 & 63.6 & 47.3\\  
			\bottomrule
		\end{tabular}
		\vspace{1mm}
		\caption{Accuracy on out-of-domain datasets.}
		\label{tab:ood}
    \end{minipage} 
\end{table}
\vspace{-7mm}

==> nips/tbl/ood.tex <==
	\begin{table*}[htbp]
		\begin{tabular}{l|c|cc}
			\toprule
			method                                 &     MNLI   & SNLI & RTE  \\
			\midrule 
			GD+GED+TSD      &     80.64    & 75.91  & 65.70 \\ 
			GD+TAD+TSD       &  80.53 & 70.93 & 52.81\\  
            GD+TSD       &   75.24 & 63.66 & 47.29\\  
			\bottomrule
		\end{tabular}
		\caption{Accuracy on out-of-domain datasets.}
		\label{tab:ood}
	\end{table*}

==> nips/tbl/task_data_ablation.tex <==
	\begin{table}[htp]
		\centering
		\scalebox{0.8}{
		\begin{tabular}{ l|ccccc } 
			\toprule
			Method & MNLIm & MNLImm                  & MRPC         &   CoLA & Avg.  \\
							\midrule

			BERT${}_{Base}$ (T.)             & 84.5 & 84.6                & 86.8                  & 61.3  & 77.4    \\
			\midrule
			ERNIE-Tiny    &83.0 & 83.0       &86.9 &  50.0 & 73.9 \\ 
			ERNIE-Tiny(w/o TAD)        &81.2 & 81.5       &     86.3   &  37.4 & 71.1\\ 
			ERNIE-Tiny(w/o TAD \& TSD) +FT   &80.7 & 81.2         &79.8 &  0^* &61.6      \\ 
			\bottomrule
		\end{tabular}
		}
		\vspace{1mm}
		\caption{Ablation study on distillation with task-specific data. FT denotes finetuning model directly. $^{*}$ The MCC of CoLA is 0 means no better than random prediction.}
		\label{tab:task_data_ablation}
	\end{table}
	
	\vspace{-7mm}
